TCN Mapping Optimization for Ultra-Low Power Time-Series Edge Inference

Temporal Convolutional Networks (TCNs) are emerging lightweight Deep Learning models for Time Series analysis. We introduce an automated exploration approach and a library of optimized kernels to map TCNs on Parallel Ultra-Low Power (PULP) microcontrollers. Our approach minimizes latency and energy by exploiting a layer tiling optimizer to jointly find the tiling dimensions and select among alternative implementations of the causal and dilated 1D-convolution operations at the core of TCNs. We benchmark our approach on a commercial PULP device, achieving up to 103X lower latency and 20.3X lower energy than the Cube-AI toolkit executed on the STM32L4 and from 2.9X to 26.6X lower energy compared to commercial closed-source and academic open-source approaches on the same hardware target.

==> text/Results_old.tex <==
\section{Experimental Results and Discussion}
\label{sec:results}
%
In this section, we first analyze our proposed 1D convolutional kernel implementations and the benefits of each of them in different scenarios. 
%
We then compare the achieved results with the state-of-the-art convolutional backends (PULP-NN~\cite{garofalo2020pulp}, GWT Autotiler~\cite{GWTAutotiler}, Cube-AI~\cite{CubeAI}) onto three hardware platforms, namely GAP-8, the STM32H7, and the STM32L4. 
%
We conclude with a complete profiling of the layers of networks for three popular use-cases, sEMG-based Gesture Recognition \cite{zanghieri2019robust}, sound generation \cite{bai2018empirical}, and language modeling \cite{bai2018empirical}.
%
\subsection{Kernels Analysis}
\label{subsec:kernel_res}
%
\input{text/Table1.tex}
%
Table~\ref{tab:perf_pulp_tcn} showcases the detailed analysis of the three implementations of the 1D convolution on two layers, the former with low channels and a long time dimension (typical of first layers of a network), and the second with high channels and smaller time dimension (typical of the end of the networks). 
%
We use only 32 out channels to fit the 44KB L1 memory of the GAP-8 processor. This kernel is one of the 8 identical tiles that are run in case of a 256$\times$16$\times$256 layer.
%

First, we observe an high degree of parallelism over the time dimension for all the three kernels (7.24$\times$ to 7.81$\times$).
%
Note that the nearly optimal parallelization is not given by a limit in the kernel parallelism -- the number of instruction is always reduced by a factor of 8 -- but to an increasing memory contention with more executing cores.
%

Then, we observed three fundamentals properties in the trade-off between our implementations.\\
%
\textit{i)} The \textbf{no-im2col kernel} is always the best for layers with dilation = 1. The layer combines the minimum number of loops in MAC execution -- we don't need to increase the input pointer buffer by factors $>$ 1, hence using always the single post-increment loads of native ISA -- without necessitating to create an additional reordering buffer (im2col).\\
%
\textit{ii)} The \textbf{im2col kernel} is usually preferable in the first layers of the networks, with a lower number of input channels. The overhead of creating the im2col, both in terms of memory overhead and execution cycles is proportional to $Ch_{in}$.
%
Noteworthy, a kernel with 256 input channels and a 3x1 filter, present a memory overhead of 12.3 KB, which is the 27.9\% of the whole available L1 memory of the GAP-8 processor. \\
%
\textit{ii)} To cope with this problem, we see that using the \textbf{indirect kernel} cause almost the same number of execution cycles for layers with many input channels, while eliminating the memory overhead.
%
In this way, for bigger layers where different layer blocks (tiles) should be executed to complete the whole computation, we can create wider and more regular tiles which present better execution performance.
%
In Section \ref{subsec:use_cases}, we will better describe the gain of using the indirect kernel for a TCN with many filters per layer.

\subsection{Comparison with GAP-8 backends and State-of-the-art edge-nodes}
\label{subsec:SoaCompare}
%
\begin{figure}
  \centering
\includegraphics[width=1\columnwidth]{./figures/Comparison_GAP8_backends}
  \caption{Comparison of our work with previous open-source and closed-source libraries on GAP8 platform.}
  \label{fig:compare}
\end{figure}
%
\input{text/Table3.tex}
%
Figure~\ref{fig:compare} depicts our proposed kernels and their comparison to the open-source PULP-NN and the commercial closed-source GWT nn-tool. 
%
In graphs A and C, we can observe a dramatically higher performance compared to the GWT nn-tool, xxx$\times$ to xxx$\times$, given that the CHW format used in the convolutions strongly disadvantage the 1D convolutions which are naturally executed as matrix multiplication with dilation = 1.
%
If compared to PULP-NN, we can observe a slightly higher performance keeping unitary dilation, thanks to the removal of unnecessary im2col creation and to the redesign of the MAC internal loop execution, while an increasing benefit while using higher dilation factors: since the PULP-NN kernels do not support this fundamental 1D-convolution propriety, the only way to have identical filters is to pad the weights with interleaving 0s, increasing the filter dimension from K to $(K-1)\times d + 1$ and hence doing many useless MACs.

Table~\ref{tab:Soa-layer} further extends this analysis, including Cube-ai backend for ARM based ST boards, state-of-the-art for ARM microcontrollers.
%
We obtain a speed-up of up to 5.6$\times$/5.8$\times$ on a single 256$\times$16$\times$256 layer executed on the STM32H7, with $\sim$28$\times$ lower number of operations at a frequency $\sim$5$\times$ lower. The energy-efficiency of the layer is up to 26.7$\times$ higher with hour implementation, strongly increasing the battery life of the smart edge-node.
%
Note that both GWT NN-Tool and Cube-AI as well as our work supports layers with flexible dilation without performance degradation, while PULP-NN strongly reduces its performance with an increasing dilation factor.
%
Further, being tailored for the execution of 1D-convolutional layers, our library takes advantage of unitary dilation to reduce the computation and yet increase the performance.
%

\subsection{Use-cases: Bio-signal and sound classification}
%
\label{subsec:use_cases}
%
\begin{figure*}
  \centering
\includegraphics[width=.8\textwidth]{./figures/ResultsUseCases}
  \caption{From left to right, we explore three TCNs architectures on three different tasks, comparing our proposed software backend with state-on-the-art. We use GAP8 for all our implementation and PULP-NN and GWT nn-tool. We run Cube-AI on STM32H7 and STM32L4 platforms.}
  \label{fig:UseCases}
\end{figure*}
%
In this section, we analyze three architectures of TCNs of variable dimensions, for three use-cases.
%
From left to right in Figure~\ref{fig:UseCases}, we observe the TEMPONet presented in \cite{zanghieri2019robust} and two TCNs from \cite{bai2018empirical}, the first for sound generation and the second for language modelling.
%
Also, from left to right the networks have an increasing number of parameters and MACs; while the layer of the networks is almost constant (9,8, and 10 layers), the number of filters per layer is increasingly high (from a maximum of 128 in the first network to 450 in the last one).
%
In details, the first network has a modular structure which progressively shrink the time dimension while increasing the number of channels up to 128~\cite{zanghieri2019robust}, while the other two architectures maintain a constant time dimension (16 and 50) with respectively 150 and 450 filters per layer.

We analyse different topologies and network dimensions to show the generality of our approach that can maintain high performance in different scenarios.
%
We observe two main findings from these results.
%
First, we see that using our model optimizer for kernel selection if compared to using a single kernel, leads to up to $4.0\times$ speed-up.
%
While implementing all the layers of the TEMPONet with im2col kernel leads to a near-optimal implementation, the same kernel for the language-modelling TCN demonstrates 4$\times$ lower performance.
%
In the same way, considering solely the indirect kernel results in $1.3\times$ lower performance on the TEMPONet execution.
%
On the different networks, we reached up to 1.2 GMACs/s, with an efficiency of 22 GMACs/s/W.
%
From these use-cases, we conclude that choosing the appropriate kernel for each layer is a key point to maximize performance: for layers with dilation = 1, the no-im2col kernel reaches the highest performance, while the im2col and the indirect ones are optimal for layers with dilation > 1 with a low/high number of channels, respectively.
%

Then, we also compare our best performance with state-of-the-art backends as presented in previous sections, but on the execution of whole TCNs.
%
For the different networks, we see a minimum speed-up of $2.9\times$ if compared to PULP-NN backend. However, 2 of the 3 networks can not be implemented using this backend given the high memory overhead of the im2col support buffer and the limited memory of the microcontroller. NON VERO -- BASTA ESEGUIRLO DA L2 DIRETTAMENTE, MA CON PERFORMANCE DISASTROSE
%
When we compare to cube-ai and GWT nn-tool on all three networks, we observe speed-ups of $2.8\times$ to $26.6\times$, with an at least $12.9\times$ better energy efficiency.
%
If we also compare to the custom implementation of the TEMPONet proposed in \cite{zanghieri2019robust}, we achieve 11.53 MAC/cycles vs 7.73 MAC/cycles, 49\% better performance with respect to the original implementation, which uses a customized version of PULP-NN for an optimal execution of the network.
%

==> text/Table1.tex <==
\begin{table*}[t]
\caption{Cycles, energy-efficiency, and memory consumption of the three implementations of 1D-convolutions. We show parallelization and speed-up on multiple rows of the table.}
\label{tab:perf_pulp_tcn}
\begin{tabular}{lp{1cm}p{1.4cm}p{1.3cm}p{1.2cm}p{1.1cm}lllp{0.7cm}p{0.7cm}p{1cm}l}
\multicolumn{1}{l|}{}    & \multicolumn{6}{c|}{Ch$_{in}$ x time x Ch$_{out}$: 32x256x32,   filter = 3, dilation = 1 (4)}                                           & \multicolumn{6}{c}{Ch$_{in}$ x time x Ch$_{out}$: 256x16x32, filter = 3,   dilation = 1 (4)}       \\
\multicolumn{1}{c|}{}    & im2col     & MACs         & Total      &             &            & \multicolumn{1}{c|}{}                & im2col     & MACs    & Total  &         &         &                 \\
\multicolumn{1}{c|}{}    & Nr. Instr. & kInstr.      & kCycles    & Speedup     & GMAC/s/W   & \multicolumn{1}{c|}{Memory {[}KB{]}} & Nr. Instr. & kInstr. & Cycles & Speedup & GMAC/s/W & Memory {[}KB{]} \\ \hline
\multicolumn{13}{l}{\textbf{PULP-TCN no-im2col}}                                                                                                                                                          \\
\multicolumn{1}{c|}{1 C} & 0 (0)      & 460 (1139)   & 472 (1158) & 1(1)x       & 9.1 (3.7)  & \multicolumn{1}{c|}{19.5 (25.6)}     & 0          & 179.3   & 181.0  & 1x      & 11.9    & 29.2 (78.3)     \\
\multicolumn{1}{c|}{2 C} & 0 (0)      & 230 (574)    & 237 (581)  & 2.0(2.0)x   & 14.9 (6.1) & \multicolumn{1}{c|}{19.5 (25.6)}     & 0          & 89.6    & 91.0   & 1.99x   & 19.4    & 29.2 (78.3)     \\
\multicolumn{1}{c|}{4 C} & 0 (0)      & 115 (287)    & 120 (292)  & 3.94(3.96)x & 20.3 (8.3) & \multicolumn{1}{c|}{19.5 (25.6)}     & 0          & 44.8    & 46.1   & 3.92x   & 26.3    & 29.2 (78.3)     \\
\multicolumn{1}{c|}{8 C} & 0 (0)      & 57.5 (143.5) & 62 (148)   & 7.62(7.81)x & 27 (11.3)  & \multicolumn{1}{c|}{19.5 (25.6)}     & 0          & 22.4    & 23.8   & 7.60x   & 35.1    & 29.2 (78.3)     \\ \hline
\multicolumn{13}{l}{\textbf{PULP-TCN im2col}}                                                                                                                                                             \\
\multicolumn{1}{c|}{1 C} & 27.8k      & 460.6       & 507.4     & 1x          & 8.5        & \multicolumn{1}{c|}{19.65}              & 7.1k       & 179.3  & 191.6 & 1x      & 11.2    & 30.7         \\
\multicolumn{1}{c|}{2 C} & 13.9k      & 230.4       & 255.2     & 1.99x       & 13.8       & \multicolumn{1}{c|}{19.84}              & 3.55k      & 89.6   & 96.3  & 1.99x   & 18.3    & 32.3        \\
\multicolumn{1}{c|}{4 C} & 7.0k       & 115.2      & 129.8     & 3.91x       & 18.7       & \multicolumn{1}{c|}{20.22}              & 1.8k       & 44.8   & 49.4  & 3.88k   & 24.6    & 35.3         \\
\multicolumn{1}{c|}{8 C} & 3.5k       & 57.6        & 68.7      & 7.39x       & 24.4       & \multicolumn{1}{c|}{20.99}              & 0.9k       & 22.4   & 26.4  & 7.27x   & 31.7    & 41.5         \\ \hline
\multicolumn{13}{l}{\textbf{PULP-TCN indirect}}                                                                                                                                                           \\
\multicolumn{1}{c|}{1 C} & 6.1k       & 571.5       & 599.9     & 1x          & 7.2        & \multicolumn{1}{c|}{19.5}            & 384        & 186.2  & 189.6 & 1x      & 11.3    & 29.2         \\
\multicolumn{1}{c|}{2 C} & 3.1k       & 285.8       & 301.5     & 1.99x       & 11.7       & \multicolumn{1}{c|}{19.5}            & 192        & 93.1   & 95.6  & 1.98x   & 18.4    & 29.2         \\
\multicolumn{1}{c|}{4 C} & 1.5k       & 142.9       & 153.8     & 3.90x       & 15.8       & \multicolumn{1}{c|}{19.5}            & 96         & 46.6   & 48.8  & 3.88x   & 24.8    & 29.2         \\
\multicolumn{1}{c|}{8 C} & 768        & 71.4        & 80.8      & 7.43x       & 20.7       & \multicolumn{1}{c|}{19.5}            & 48         & 23.3   & 26.2  & 7.24x   & 31.9    & 29.2         \\ \hline
\end{tabular}
\end{table*}

==> text/Table3.tex <==

\begin{table}[t]
\centering
\begin{threeparttable}
\caption{Detailed performance and energy efficiency on a 256x16x32 ($C_{in}\times T \times C_{out}$) layer, with $K = 3$ and dilation $d = 1$ or $2$.}
\label{tab:Soa-layer}
{
\centering
\footnotesize
%\setlength\arrayrulewidth{1pt}
\renewcommand{\arraystretch}{1.2}
\setlength\tabcolsep{5pt}
\begin{tabular}{cc|c|c|c}
&  & \multicolumn{2}{c|}{\textbf{Performance (speed-up)}}        & \textbf{Efficiency}  \\                            
Work & Dilation &  MAC/cycle             &   GMAC/s               &   GMAC/s/W           \\ \hline\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Our Work\tnote{a}}\end{tabular}}} & d = 1 & 16.6 (1$\times$)     & 1.7 (1$\times$)    & 32.6 (1$\times$)      \\ \cline{2-5} 
\multicolumn{1}{c|}{}   & d = 2 & 16.1 (1$\times$)     & 1.6 (1$\times$)    & 31.6 (1$\times$)      \\ \hline\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{PULP-NN \cite{garofalo2020pulp}\tnote{a}}\end{tabular}}} & d = 1 & 15.8 (1.05$\times$)     & 1.6 (1.05$\times$)    & 30.9 (1.05$\times$)      \\ \cline{2-5} 
\multicolumn{1}{c|}{}   & d = 2 & 9.7 (1.7$\times$)     & 1.0 (1.7$\times$)    & 19.1 (1.7$\times$)      \\ \hline\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{GWT NN-Tool \cite{GWTAutotiler}\tnote{a}}\end{tabular}}} & d = 1 & 1.1 (15.3$\times$)     & 0.1 (15.3$\times$)    & 2.1 (15.3$\times$)      \\ \cline{2-5} 
\multicolumn{1}{c|}{}   & d = 2 & 1.1 (14.8$\times$)     & 0.1 (14.8$\times$)    & 2.1 (14.8$\times$)      \\ \hline\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Cube-AI \cite{CubeAI}\tnote{b}}\end{tabular}}} & d = 1 & 0.6 (27.9$\times$)     & 0.3 (5.8$\times$)    & 1.2 (26.7$\times$)        \\ \cline{2-5} 
\multicolumn{1}{c|}{}   & d = 2 & 0.6 (27.1$\times$)     & 0.3 (5.6$\times$)    & 1.2 (25.9$\times$)      \\ \hline\hline
\end{tabular}
}
\begin{tablenotes}
\item [a] Collected on the GWT GAP8 @ (100MHz, 1.0V).
\item [b] Collected on the STM32H7 @ (480MHz, 3.3V).
\end{tablenotes}
\end{threeparttable}
\vspace{-0.6cm}
\end{table}

==> text/backup.tex <==

\subsection{Quantization}
\label{subsec:qnn}

Accordingly, our proposed kernels focus on 8-bit QNNs.
%
In particular, we rely on the open-source NEMO tool~\cite{conti2020nemo} to generate quantized TCN topologies using a linear, layer-wise quantization.
% 
\textbf{Sposterei nei methods}

\subsection{Target Platform}
\label{subsec:platform}
\begin{figure}
  \centering
\includegraphics[width=0.995\columnwidth]{./figures/gap8.pdf}
  \caption{GWT GAP-8 MCU block diagram.}
\label{fig:GAP8}
\end{figure}
PULP (Parallel Ultra-Low Power) is an architectural paradigm leveraging near-threshold computing to achieve high energy efficiency, coupled with parallelism to improve the performance degradation at low-voltage. Figure~\ref{fig:GAP8} depicts GWT GAP-8~\cite{flamand2018gap}, a commercial embodiment of PULP, which is the reference platform used in this work for our experiments. It consists of a state-of-the-art microcontroller system (\textit{SoC domain}) built around a controlling processor (\textit{fabric controller}) and a standard set of peripherals, offloading parallel tasks to a software-programmable parallel accelerator composed of 8 additional RISC-V cores, standing in it own voltage and frequency domain (\textit{cluster domain}).

The cores within the cluster are 4-stage in-order single-issue pipelines called RI5CY~\cite{gautschi2017near}, implementing the RISC-V RV32IMCXpulpV2 Instruction Set Architecture (ISA). XpulpV2 is a domain-specific extension meant for efficient digital signal processing, with hardware loops, post-modified access LD/ST, and SIMD instructions down to 8-bit vector operands. The 8 cores of the \textit{cluster} share a 64 kB multi-banked L1 memory Tightly-Coupled Data Memory (TCDM), accessible from the cluster's cores through a high-bandwidth, single-cycle-latency logarithmic interconnect, featuring a 2x banking factor and a word-level interleaving scheme to reduce the probability of contention~\cite{rahimi2011fully}.  \textbf{DA SPOSTARE NELL'EXPERIMENTAL SETUP}

==> text/biblioCompressed.tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{zanghieri2019robust}
M.~Zanghieri \emph{et~al.}, ``Robust real-time embedded emg recognition
  framework using temporal convolutional networks on a multicore iot
  processor,'' \emph{IEEE TBioCAS}, vol. 14, no. 2, pp. 244-256, 2019.

\bibitem{burrello2020enhancing}
A.~Burrello \emph{et~al.}, ``Enhancing structural health monitoring with
  vehicle identification and tracking,'' in \emph{Proc. of the IEEE I2MTC}, 2020, pp. 1--6.

\bibitem{palossi201964mw}
D.~Palossi \emph{et~al.}, ``A 64mw dnn-based visual navigation engine for
  autonomous nano-drones,'' \emph{IEEE IOT-J}, vol. 6, no. 5, pp. 8357-8371, 2019.

\bibitem{flamand2018gap}
E.~Flamand \emph{et~al.}, ``Gap-8: A risc-v soc for ai at the edge of the
  iot,'' in \emph{Proc. of the 29th IEEE ASAP}, 2018, pp. 1--4.

\bibitem{shangguan2019optimizing}
Y.~Shangguan \emph{et~al.}, ``Optimizing speech recognition for the edge,''
  2019.

\bibitem{bai2018empirical}
S.~Bai \emph{et~al.}, ``An empirical evaluation of generic convolutional and recurrent networks for sequence modeling,'' \emph{arXiv preprint
  arXiv:1803.01271}, 2018.

\bibitem{ren2020cloud}
L.~Ren \emph{et~al.}, ``Cloud-edge based lightweight temporal convolutional
  networks for remaining useful life prediction in iiot,'' \emph{IEEE IOT-J}, 2020.

\bibitem{lea2016temporal}
C.~Lea \emph{et~al.}, ``Temporal convolutional networks: A unified approach to
  action segmentation,'' in \emph{Proc. of ECCV}, 2016, pp. 47--54.

\bibitem{st-dual}
\BIBentryALTinterwordspacing
STMicroelectornics. STM32H7. [Online]. Available:
  \url{https://www.st.com/en/microcontrollers-microprocessors/stm32h7-series.html}
\BIBentrySTDinterwordspacing

\bibitem{nxp}
\BIBentryALTinterwordspacing
NXP. NXP LPC4300. [Online]. Available:
  \url{https://www.nxp.com/products/processors-and-microcontrollers/arm-microcontrollers/general-purpose-mcus/lpc4300-cortex-m4-m0}
\BIBentrySTDinterwordspacing

\bibitem{TPU}
\BIBentryALTinterwordspacing
N.~P. Jouppi \emph{et~al.}, ``In-datacenter performance analysis of a tensor
  processing unit,'' in \emph{Proce. of the 44th ACM ISCA}, 2017, p. 1–12.

\bibitem{garofalo2020pulp}
A.~Garofalo \emph{et~al.}, ``Pulp-nn: accelerating quantized neural networks on
  parallel ultra-low-power risc-v processors,'' \emph{Philos. Trans. R. Soc. A}, vol. 378, no. 2164, p. 20190155, 2020.

\bibitem{lai2018cmsis}
L.~Lai \emph{et~al.}, ``Cmsis-nn: Efficient neural network kernels for arm
  cortex-m cpus,'' \emph{arXiv preprint arXiv:1801.06601}, 2018.

\bibitem{wang2020fann}
X.~Wang \emph{et~al.}, ``Fann-on-mcu: An open-source toolkit for energy-efficient neural network inference at the edge of the internet of things,'' \emph{IEEE IOT-J}, vol. 7, no. 5, pp. 4403-4417, 2020.

\bibitem{GWTAutotiler}
\BIBentryALTinterwordspacing
GWT. (2019) Gap8 NN-Tool. [Online]. Available:
  \url{https://greenwaves-technologies.com/manuals/build/autotiler/html/index.html}
\BIBentrySTDinterwordspacing

\bibitem{gautschi2017near}
M.~Gautschi \emph{et~al.}, ``Near-threshold risc-v core with dsp extensions for
  scalable iot endpoint devices,'' \emph{IEEE TVLSI}, vol.~25, pp. 2700--2713, 2017.

\bibitem{CubeAI}
\BIBentryALTinterwordspacing
STMicroelectornics. (2017) X-cube-ai. [Online]. Available:
  \url{https://www.st.com/en/embedded-software/x-cube-ai.html}
\BIBentrySTDinterwordspacing

\bibitem{burrello2020dory}
A.~Burrello \emph{et~al.}, ``Dory: Automatic end-to-end deployment of
  real-world dnns on low-cost iot mcus,'' \emph{arXiv preprint arXiv:2008.07127}, 2020.

\bibitem{dukhan2019indirect}
M.~Dukhan, ``The indirect convolution algorithm,'' \emph{arXiv preprint arXiv:1907.02129}, 2019.

\bibitem{rahimi2011fully}
A.~Rahimi \emph{et~al.}, ``A fully-synthesizable single-cycle interconnection
  network for shared-l1 processor clusters,'' in \emph{Proc. of DATE}, 2011, pp. 1--6.

\end{thebibliography}

